Network Contention State Aware Dynamic Optimizer for Accelerator Collective Communication Libraries

Collective Communication Libraries (CCL) are critical for large-scale distributed AI/ML training, yet their configurations are determined by static heuristics that do not account for real-time network conditions. Our empirical study shows that these heuristics perform near-optimally in contention-free environments, but degrade substantially under background traffic. To address this, we present a cooperative multi-agent run-time optimizer for accelerator collective communication. Our approach employs a two-agent architecture: (i) detector- a Long Short Term Memory(LSTM) recurring neural network fed classifier head with a sequential probability ratio test that distinguishes sustained contention from transient spikes; and (ii) selector- a configuration selector built on a Dueling Double DQN (D3QN) with Conservative Q-Learning that adapts configuration parameters in response. We implemented this dynamic tuner over NCCL, a widely used CCL developed by NVIDIA. When evaluated on Chameleon Cloud's isolated bare-metal cluster, this dynamic tuning approach reduces AllReduce latency by 36% over NCCL and 32% over a fully converged AutoCCL. We further evaluated it across six real AI workloads spanning convolutional networks, transformers, and recommendation architectures. Our multi-agent tuner approach delivers up to 65% speedups on Delta cluster with NVIDIA A100 GPUs and Slingshot-11 fabric internode connectivity.

==> figures/coord_timeline.tex <==
% \begin{tikzpicture}[font=\Large, node distance=0.5cm, xscale=1.0, yscale=1.2]

%   % Column headers
%   \node[align=center, font=\bfseries] (p1) at (0, 0)   {NCCL Rank\\(Plugin)};
%   \node[align=center, font=\bfseries] (p2) at (4, 0)   {Coordinator\\(Skeleton)};
%   \node[align=center, font=\bfseries] (p3) at (8, 0)   {Optimizer\\(KV Cache)};
%   \node[align=center, font=\bfseries] (p4) at (12, 0)  {Agent Chain\\(Async)};

%   % Lifelines
%   \foreach \x in {0, 4, 8, 12}
%     \draw[dashed, gray, ultra thick] (\x, -0.3) -- (\x, -10.5);

%   % === CRITICAL PATH ===
%   \node[draw, fill=yellow!20, align=center, font=\footnotesize]
%     at (6, -0.9) {$\equiv$ BEGIN CRITICAL PATH $\equiv$};

%   % AllReduce(N) arrives
%   \draw[->, thick] (0,-1.4) -- (4,-1.4)
%     node[midway, above, font=\footnotesize] {AllReduce($N$)};

%   % GetCollInfo
%   \draw[->, thick] (4,-1.9) -- (8,-1.9)
%     node[midway, above, font=\footnotesize] {GetCollInfo()};

%   % process(): KV lookup
%   \draw[thick] (8,-2.2) -- (8,-2.8);
%   \node[right, font=\footnotesize, align=left] at (8.1,-2.5)
%     {(a) \texttt{process(info)}\\KV cache lookup O(1)};

%   % Config C reply
%   \draw[->, thick] (8,-3.1) -- (4,-3.1)
%     node[midway, above, font=\footnotesize] {Config $C$};
%   \draw[->, thick] (4,-3.4) -- (0,-3.4)
%     node[midway, above, font=\footnotesize] {TCP reply};

%   \node[draw, fill=yellow!20, align=center, font=\footnotesize]
%     at (6, -3.8) {$\equiv$ END CRITICAL PATH $\equiv$};

%   % AllReduce(N) executes
%   \node[font=\footnotesize, align=center] at (2, -4.3)
%     {AllReduce($N$) executes\\with Config $C$};
%   \draw[thick] (0,-4.0) -- (4,-4.0);

%   % read_all_latest
%   \draw[thick] (8,-4.6) -- (8,-5.2);
%   \node[right, font=\footnotesize, align=left] at (8.1,-4.9)
%     {\texttt{read\_all\_latest()}\\$\rightarrow$ GPUStats from shm\\$\rightarrow$ \texttt{coll\_latency} of $N$-1};

%   % observe()
%   \draw[thick] (8,-5.5) -- (8,-6.1);
%   \node[right, font=\footnotesize, align=left] at (8.1,-5.8)
%     {(b) \texttt{observe(info, cfg, stats)}\\update snapshot\\++\texttt{counter\_k}};

%   % trigger agent chain
%   \draw[->, dashed] (8,-6.6) -- (12,-6.6)
%     node[midway, above, font=\footnotesize] {trigger?};

%   % fwd+bwd pass overlap
%   \draw[thick, fill=blue!10] (0,-6.6) rectangle (3.8,-8.4);
%   \node[font=\footnotesize, align=center] at (1.9,-7.5)
%     {fwd pass\\bwd pass\\(100ms -- seconds)};

%   % Agent-1 + Agent-2
%   \draw[thick] (12,-6.6) -- (12,-8.4);
%   \node[right, font=\footnotesize, align=left] at (12.1,-7.0)
%     {Agent-1: LSTM tick};
%   \node[right, font=\footnotesize, align=left] at (12.1,-7.5)
%     {$\rightarrow$ CONG or CLEAN:};
%   \node[right, font=\footnotesize, align=left] at (12.1,-8.0)
%     {Agent-2: DQN infer\\$\rightarrow$ write KV cache\\$\rightarrow$ reset triggers};

%   % return from agent chain
%   \draw[->, dashed] (12,-8.5) -- (8,-8.5);

%   % AllReduce(N+1) arrives
%   \draw[->, thick] (0,-9.0) -- (4,-9.0)
%     node[midway, above, font=\footnotesize] {AllReduce($N$+1)};

%   \draw[->, thick] (4,-9.3) -- (8,-9.3)
%     node[midway, above, font=\footnotesize] {GetCollInfo()};

%   \draw[thick] (8,-9.6) -- (8,-10.0);
%   \node[right, font=\footnotesize, align=left] at (8.1,-9.8)
%     {(a) \texttt{process(info)}\\$\rightarrow$ Config $C'$ (updated)};

%   \draw[->, thick] (8,-10.2) -- (4,-10.2)
%     node[midway, above, font=\footnotesize] {Config $C'$};

% \end{tikzpicture}


\begin{tikzpicture}[font=\large, node distance=0.5cm, xscale=1.0, yscale=1.2,
                    >=latex, line width=1pt]

  % Column headers
  \node[align=center, font=\large\bfseries] (p1) at (0, 0)   {NCCL Rank\\(Plugin)};
  \node[align=center, font=\large\bfseries] (p2) at (4, 0)   {Coordinator\\(Skeleton)};
  \node[align=center, font=\large\bfseries] (p3) at (8, 0)   {Optimizer\\(KV Cache)};
  \node[align=center, font=\large\bfseries] (p4) at (12, 0)  {Agent Chain\\(Async)};

  % Lifelines -- thicker, darker
  \foreach \x in {0, 4, 8, 12}
    \draw[dashed, black!60, line width=1.2pt] (\x, -0.3) -- (\x, -10.5);

  % === CRITICAL PATH ===
  \node[draw, fill=yellow!20, align=center, font=\normalsize\bfseries,
        line width=1pt, inner sep=4pt]
    at (6, -0.9) {$\equiv$ BEGIN CRITICAL PATH $\equiv$};

  % AllReduce(N) arrives
  \draw[->, line width=1.4pt] (0,-1.4) -- (4,-1.4)
    node[midway, above, font=\normalsize] {AllReduce($N$)};

  % GetCollInfo
  \draw[->, line width=1.4pt] (4,-1.9) -- (8,-1.9)
    node[midway, above, font=\normalsize] {GetCollInfo()};

  % process(): KV lookup
  \draw[line width=1.4pt] (8,-2.2) -- (8,-2.8);
  \node[right, font=\normalsize, align=left] at (8.15,-2.5)
    {(a) \texttt{process(info)}\\KV cache lookup O(1)};

  % Config C reply
  \draw[->, line width=1.4pt] (8,-3.1) -- (4,-3.1)
    node[midway, above, font=\normalsize] {Config $C$};
  \draw[->, line width=1.4pt] (4,-3.4) -- (0,-3.4)
    node[midway, above, font=\normalsize] {TCP reply};

  \node[draw, fill=yellow!20, align=center, font=\normalsize\bfseries,
        line width=1pt, inner sep=4pt]
    at (6, -3.8) {$\equiv$ END CRITICAL PATH $\equiv$};

  % AllReduce(N) executes
  \node[font=\normalsize, align=center] at (2, -4.3)
    {AllReduce($N$) executes\\with Config $C$};
  \draw[line width=1.4pt] (0,-4.0) -- (4,-4.0);

  % read_all_latest
  \draw[line width=1.4pt] (8,-4.6) -- (8,-5.2);
  \node[right, font=\normalsize, align=left] at (8.15,-4.9)
    {\texttt{read\_all\_latest()}\\$\rightarrow$ GPUStats from shm\\$\rightarrow$ \texttt{coll\_latency} of $N{-}1$};

  % observe()
  \draw[line width=1.4pt] (8,-5.5) -- (8,-6.1);
  \node[right, font=\normalsize, align=left] at (8.15,-5.8)
    {(b) \texttt{observe(info, cfg, stats)}\\update snapshot\\++\texttt{counter\_k}};

  % trigger agent chain
  \draw[->, dashed, line width=1.4pt] (8,-6.6) -- (12,-6.6)
    node[midway, above, font=\normalsize] {trigger?};

  % fwd+bwd pass overlap
  \draw[line width=1.4pt, fill=blue!10] (0,-6.6) rectangle (3.8,-8.4);
  \node[font=\normalsize, align=center] at (1.9,-7.5)
    {fwd pass\\bwd pass\\(100ms -- seconds)};

  % Agent-1 + Agent-2
  \draw[line width=1.4pt] (12,-6.6) -- (12,-8.4);
  \node[right, font=\normalsize, align=left] at (12.15,-7.0)
    {Agent-1: LSTM tick};
  \node[right, font=\normalsize, align=left] at (12.15,-7.5)
    {$\rightarrow$ CONG or CLEAN:};
  \node[right, font=\normalsize, align=left] at (12.15,-8.5)
    {Agent-2: DQN infer\\$\rightarrow$ write KV cache\\$\rightarrow$ reset triggers};

  % return from agent chain
  \draw[->, dashed, line width=1.4pt] (12,-8.5) -- (8,-8.5);

  % AllReduce(N+1) arrives
  \draw[->, line width=1.4pt] (0,-9.0) -- (4,-9.0)
    node[midway, above, font=\normalsize] {AllReduce($N{+}1$)};

  \draw[->, line width=1.4pt] (4,-9.3) -- (8,-9.3)
    node[midway, above, font=\normalsize] {GetCollInfo()};

  \draw[line width=1.4pt] (8,-9.6) -- (8,-10.0);
  \node[right, font=\normalsize, align=left] at (8.15,-9.8)
    {(a) \texttt{process(info)}\\$\rightarrow$ Config $C'$ (updated)};

  \draw[->, line width=1.4pt] (8,-10.2) -- (4,-10.2)
    node[midway, above, font=\normalsize] {Config $C'$};

\end{tikzpicture}

==> figures/dccl_arch_tkz.tex <==
%% DynamICCL Architecture — TikZ/PGF
%% Required packages in preamble:
%%   \usepackage{tikz}
%%   \usepackage{xcolor}
%%   \usetikzlibrary{arrows.meta, shapes.geometric, positioning, fit, backgrounds, calc}
%%
%% Usage: \input{dynamiccl_arch_tikz.tex}
%% The figure scales to \linewidth automatically via the tikzpicture scale.
%% To adjust size: change \def\sc{0.155} below.

\def\sc{0.155} %% global scale: 1 SVG px = \sc pt

%% ── Color definitions ──────────────────────────────────────────
\definecolor{ddpFill}{HTML}{FEF3C7}
\definecolor{ddpBorder}{HTML}{D97706}
\definecolor{node0Fill}{HTML}{F0FDF4}
\definecolor{node0Border}{HTML}{6EE7B7}
\definecolor{ddpProcFill}{HTML}{DCFCE7}
\definecolor{ddpProcBorder}{HTML}{86EFAC}
\definecolor{gpuMonFill}{HTML}{FEF9C3}
\definecolor{gpuMonBorder}{HTML}{FDE047}
\definecolor{gpuPlugFill}{HTML}{DBEAFE}
\definecolor{gpuPlugBorder}{HTML}{93C5FD}
\definecolor{plugLdrFill}{HTML}{EDE9FE}
\definecolor{plugLdrBorder}{HTML}{A78BFA}
\definecolor{plugWrkFill}{HTML}{F1F5F9}
\definecolor{plugWrkBorder}{HTML}{CBD5E1}
\definecolor{shmFill}{HTML}{FFF7ED}
\definecolor{shmBorder}{HTML}{FB923C}
\definecolor{skelFill}{HTML}{D1FAE5}
\definecolor{skelBorder}{HTML}{34D399}
\definecolor{agent1Fill}{HTML}{FFEDD5}
\definecolor{agent1Border}{HTML}{FB923C}
\definecolor{agent2Fill}{HTML}{FCE7F3}
\definecolor{agent2Border}{HTML}{F472B6}
\definecolor{kvFill}{HTML}{F1F5F9}
\definecolor{kvBorder}{HTML}{94A3B8}
\definecolor{csockFill}{HTML}{DBEAFE}
\definecolor{csockBorder}{HTML}{93C5FD}
\definecolor{csockStubFill}{HTML}{ECFDF5}
\definecolor{csockStubBorder}{HTML}{6EE7B7}
\definecolor{stubFill}{HTML}{F1F5F9}
\definecolor{stubBorder}{HTML}{CBD5E1}
\definecolor{legendFill}{HTML}{F8FAFC}
\definecolor{legendBorder}{HTML}{E2E8F0}
\definecolor{arrowOrange}{HTML}{D97706}
\definecolor{arrowBlue}{HTML}{2563EB}
\definecolor{arrowRed}{HTML}{DC2626}
\definecolor{arrowGreen}{HTML}{059669}
\definecolor{arrowGray}{HTML}{6B7280}
\definecolor{arrowNccl}{HTML}{94A3B8}
\definecolor{textDark}{HTML}{1E293B}
\definecolor{textMid}{HTML}{374151}
\definecolor{textLight}{HTML}{6B7280}

%% ── TikZ styles ────────────────────────────────────────────────
\tikzset{
  darch/.style={
    draw, rounded corners=\sc*8 pt,
    line width=0.6pt,
    font=\sffamily\small
  },
  stepbadge/.style={
    circle, minimum size=\sc*22 pt,
    inner sep=0pt,
    font=\sffamily\bfseries\footnotesize,
    text=white
  },
  alabel/.style={font=\sffamily\tiny, text=textLight},
  boldlabel/.style={font=\sffamily\bfseries\scriptsize, text=textDark},
  smlabel/.style={font=\sffamily\scriptsize, text=textMid},
  xslabel/.style={font=\sffamily\tiny, text=textLight},
  nodelabel/.style={font=\sffamily\bfseries\scriptsize, text=textDark},
}

\begin{tikzpicture}[
  x=1pt, y=-1pt,   %% y is flipped so SVG y-down matches TikZ
  every node/.style={inner sep=2pt},
  scale=2\sc,
  transform shape
]

%% ── PyTorch DDP Training ────────────────────────────────────────
\draw[darch, fill=ddpFill, draw=ddpBorder, rounded corners=8pt]
  (325,12) rectangle (575,60);
\node[boldlabel] at (450,31) {PyTorch DDP Training};
\node[smlabel]   at (450,48) {torchrun · user code};

%% DDP → Node0 arrow (step 1)
\draw[-{Stealth[length=5pt]}, arrowOrange, line width=1.2pt]
  (380,60) -- (230,100);
%% DDP → Node1 arrow (step 1)
\draw[-{Stealth[length=5pt]}, arrowOrange, line width=1.2pt]
  (520,60) -- (670,100);
%% Step 1 badge
\node[stepbadge, fill=arrowOrange] at (298,79) {1};

%% ═══════════════════════════════════════════════════════════════
%% NODE 0
%% ═══════════════════════════════════════════════════════════════
\draw[darch, fill=node0Fill, draw=node0Border, rounded corners=12pt, line width=1.2pt]
  (16,92) rectangle (428,612);
\node[nodelabel] at (222,114) {Node 0 — Skeleton · MPI rank 0};

%% DDP process boundary (dashed)
\draw[darch, fill=ddpProcFill, draw=ddpProcBorder, dashed, rounded corners=8pt, line width=0.8pt]
  (28,122) rectangle (416,354);
\node[xslabel, anchor=west] at (44,138) {PyTorch DDP training process};

%% GPU Monitor
\draw[darch, fill=gpuMonFill, draw=gpuMonBorder, rounded corners=7pt]
  (38,146) rectangle (168,218);
\node[boldlabel] at (103,166) {GPU Monitor};
\node[smlabel]   at (103,182) {Python · NVML};
\node[smlabel]   at (103,196) {100\,ms sampling};
\node[xslabel]   at (103,210) {GPU stats + latency};

%% GPU+Plugin block
\draw[darch, fill=gpuPlugFill, draw=gpuPlugBorder, rounded corners=7pt]
  (186,146) rectangle (404,244);
\node[smlabel] at (295,165) {NCCL runtime · ncclTunerPlugin};

%% Plugin rank 0
\draw[darch, fill=plugLdrFill, draw=plugLdrBorder, rounded corners=5pt]
  (196,172) rectangle (288,212);
\node[boldlabel] at (242,187) {Plugin rank 0};
\node[xslabel]   at (242,201) {LEADER};

%% Plugin rank 1
\draw[darch, fill=plugWrkFill, draw=plugWrkBorder, rounded corners=5pt]
  (304,172) rectangle (396,212);
\node[boldlabel] at (350,187) {Plugin rank 1};
\node[xslabel]   at (350,201) {WORKER};

%% Step 2 badge
\node[stepbadge, fill=arrowRed] at (38,142) {2};

%% GPU Monitor → SHM arrow
\draw[-{Stealth[length=5pt]}, arrowRed, line width=1.2pt]
  (103,218) -- (103,250);

%% SHM block (dashed border)
\draw[darch, fill=shmFill, draw=shmBorder, dashed, rounded corners=7pt, line width=1.2pt]
  (38,250) rectangle (168,340);
\node[boldlabel] at (103,270) {Zero-Copy SHM};
\node[smlabel]   at (103,285) {POSIX · lock-free R/W};
\node[smlabel]   at (103,299) {Circ.\ buf rank 0};
\node[smlabel]   at (103,313) {Circ.\ buf rank 1};
\node[xslabel]   at (103,329) {1\,024 slots $\times$ 64\,B each};

%% Step 3a badge
\node[stepbadge, fill=arrowOrange] at (38,246) {3};

%% SHM → coordinator mmap arrow (dashed)
\draw[-{Stealth[length=5pt]}, arrowOrange, dashed, line width=1.2pt]
  (103,340) -- (103,390);
\node[alabel, anchor=west] at (108,367) {mmap};

%% Step 3b badge
\node[stepbadge, fill=arrowBlue] at (402,246) {3};

%% Plugin LEADER → coordinator arrow (TCP)
\draw[-{Stealth[length=5pt]}, arrowBlue, line width=1.2pt]
  (242,212) -- (242,390);
\node[alabel, anchor=west] at (247,310) {TCP};
\node[alabel, anchor=west] at (247,322) {collInfo};

%% ── Skeleton Coordinator ──────────────────────────────────────
\draw[darch, fill=skelFill, draw=skelBorder, rounded corners=8pt, line width=1.2pt]
  (28,390) rectangle (416,594);
\node[nodelabel] at (222,412) {Skeleton Coordinator · MPI rank 0};

%% Step 4 badge
\node[stepbadge, fill=arrowGreen] at (402,386) {4};

%% Agent-1 (Congestion Detector)
\draw[darch, fill=agent1Fill, draw=agent1Border, rounded corners=6pt]
  (196,422) rectangle (404,478);
\node[boldlabel] at (300,442) {Congestion Detector};
\node[smlabel]   at (300,458) {Agent-1-CD · LSTM + SPRT};
\node[xslabel]   at (300,472) {detect SUSTAINED / SPIKE / STEADY-STATE};

%% h_t arrow Agent-1 → Agent-2
\draw[-{Stealth[length=5pt]}, arrowRed, line width=1.2pt]
  (196,450) -- (158,450);
\node[alabel] at (177,443) {$h_t$};

%% Agent-2 (Config Selector)
\draw[darch, fill=agent2Fill, draw=agent2Border, rounded corners=6pt]
  (38,422) rectangle (190,478);
\node[boldlabel] at (114,442) {Config Selector};
\node[smlabel]   at (114,458) {Agent-2-OCS};
\node[xslabel]   at (114,472) {Dueling DQN · CPU-only · ${<}$2\,ms};

%% Agent-2 → KV Cache arrow
\draw[-{Stealth[length=5pt]}, arrowRed, line width=1.2pt]
  (114,478) -- (114,502);
\node[alabel, anchor=west] at (118,492) {update};

%% KV Cache
\draw[darch, fill=kvFill, draw=kvBorder, rounded corners=6pt]
  (38,502) rectangle (190,542);
\node[boldlabel] at (114,519) {KV Cache};
\node[xslabel]   at (114,533) {O(1) lookup · (collType, nBytes) key};

%% KV cache → CoordSocket arrow
\draw[-{Stealth[length=5pt]}, arrowBlue, line width=1.2pt]
  (190,522) -- (210,522);

%% CoordSocket local ranks
\draw[darch, fill=csockFill, draw=csockBorder, rounded corners=6pt]
  (210,502) rectangle (404,542);
\node[boldlabel] at (307,519) {CoordSocket · local ranks};
\node[xslabel]   at (307,533) {TCP reply $\to$ config inject to plugins};

%% Step 6 badge (Node 0 side)
\node[stepbadge, fill=arrowBlue] at (402,498) {6};

%% CoordSocket stubs (MPI_Bcast outgoing)
\draw[darch, fill=csockStubFill, draw=csockStubBorder, rounded corners=6pt]
  (210,556) rectangle (404,586);
\node[smlabel] at (307,575) {CoordSocket · stubs $\to$ MPI\_Bcast};

%% Step 7 feedback arrow (dashed, left side of node 0)
\draw[-{Stealth[length=5pt]}, arrowGray, dashed, line width=0.8pt]
  (38,522) -- (16,522) -- (16,190) -- (186,190);
\node[stepbadge, fill=arrowGray] at (16,356) {7};

%% ═══════════════════════════════════════════════════════════════
%% NODE 1
%% ═══════════════════════════════════════════════════════════════
\draw[darch, fill=node0Fill, draw=node0Border, rounded corners=12pt, line width=1.2pt]
  (472,92) rectangle (884,612);
\node[nodelabel] at (678,114) {Node 1\ldots N — Stub · MPI rank 1+};

%% DDP process boundary node 1 (dashed)
\draw[darch, fill=ddpProcFill, draw=ddpProcBorder, dashed, rounded corners=8pt, line width=0.8pt]
  (484,122) rectangle (872,354);
\node[xslabel, anchor=west] at (500,138) {PyTorch DDP training process};

%% GPU Monitor node 1
\draw[darch, fill=gpuMonFill, draw=gpuMonBorder, rounded corners=7pt]
  (730,146) rectangle (860,218);
\node[boldlabel] at (795,166) {GPU Monitor};
\node[smlabel]   at (795,182) {Python · NVML};
\node[smlabel]   at (795,196) {100\,ms sampling};
\node[xslabel]   at (795,210) {GPU stats + latency};

%% GPU+Plugin block node 1
\draw[darch, fill=gpuPlugFill, draw=gpuPlugBorder, rounded corners=7pt]
  (484,146) rectangle (702,244);
\node[smlabel] at (593,165) {NCCL runtime · ncclTunerPlugin};
\draw[darch, fill=plugLdrFill, draw=plugLdrBorder, rounded corners=5pt]
  (494,172) rectangle (586,212);
\node[boldlabel] at (540,187) {Plugin rank 2};
\node[xslabel]   at (540,201) {LEADER};
\draw[darch, fill=plugWrkFill, draw=plugWrkBorder, rounded corners=5pt]
  (602,172) rectangle (694,212);
\node[boldlabel] at (648,187) {Plugin rank 3};
\node[xslabel]   at (648,201) {WORKER};

%% Step 2 badge node 1
\node[stepbadge, fill=arrowRed] at (730,142) {2};
\draw[-{Stealth[length=5pt]}, arrowRed, line width=1.2pt]
  (795,218) -- (795,250);

%% SHM node 1
\draw[darch, fill=shmFill, draw=shmBorder, dashed, rounded corners=7pt, line width=1.2pt]
  (730,250) rectangle (860,340);
\node[boldlabel] at (795,270) {Zero-Copy SHM};
\node[smlabel]   at (795,285) {POSIX · lock-free R/W};
\node[smlabel]   at (795,299) {Circ.\ buf rank 2};
\node[smlabel]   at (795,313) {Circ.\ buf rank 3};
\node[xslabel]   at (795,329) {1\,024 slots $\times$ 64\,B each};

%% Stub Coordinator
\draw[darch, fill=stubFill, draw=stubBorder, rounded corners=8pt, line width=1.2pt]
  (484,390) rectangle (872,594);
\node[nodelabel] at (678,412) {Stub Coordinator · MPI rank 1+};
\node[smlabel]   at (678,448) {no optimizer · no agents};
\node[smlabel]   at (678,466) {receives config via MPI\_Bcast};
\node[smlabel]   at (678,484) {forwards to local ranks via TCP};

%% CoordSocket local ranks stub
\draw[darch, fill=csockFill, draw=csockBorder, rounded corners=6pt]
  (506,502) rectangle (854,542);
\node[boldlabel] at (680,519) {CoordSocket · local ranks};
\node[xslabel]   at (680,533) {TCP reply $\to$ config inject to plugins};

%% Step 6 badge stub side
\node[stepbadge, fill=arrowBlue] at (484,498) {6};

%% Stub → plugins feedback (step 7, dashed right side)
\draw[-{Stealth[length=5pt]}, arrowGray, dashed, line width=0.8pt]
  (856,502) -- (876,502) -- (876,190) -- (702,190);
\node[stepbadge, fill=arrowGray] at (876,356) {7};

%% CoordSocket stubs receive
\draw[darch, fill=csockStubFill, draw=csockStubBorder, rounded corners=6pt]
  (506,556) rectangle (854,586);
\node[smlabel] at (680,575) {CoordSocket · stubs $\leftarrow$ MPI\_Bcast};

%% ═══════════════════════════════════════════════════════════════
%% INTER-NODE CONNECTIONS
%% ═══════════════════════════════════════════════════════════════

%% NCCL transport (dashed, bidirectional)
\draw[-{Stealth[length=5pt]}, arrowNccl, dashed, line width=1pt]
  (428,182) -- (472,182);
\draw[-{Stealth[length=5pt]}, arrowNccl, dashed, line width=1pt]
  (472,196) -- (428,196);
\node[alabel] at (450,176) {NCCL};
\node[alabel] at (450,204) {transport};

%% MPI_Bcast inter-node (step 5)
\draw[-{Stealth[length=7pt]}, arrowGreen, line width=2pt]
  (428,571) -- (506,571);
\node[stepbadge, fill=arrowGreen] at (450,557) {5};
\node[alabel, anchor=west] at (467,551) {MPI\_Bcast};
\node[alabel, anchor=west] at (467,563) {5 $\times$ uint32};

%% ═══════════════════════════════════════════════════════════════
%% LEGEND
%% ═══════════════════════════════════════════════════════════════
\draw[darch, fill=legendFill, draw=legendBorder, rounded corners=10pt, line width=0.8pt]
  (16,628) rectangle (884,768);

%% Color guide title
\node[font=\sffamily\bfseries\scriptsize, text=textDark, anchor=west] at (30,650) {Color guide};

%% Row 1 swatches
\draw[fill=node0Fill,  draw=node0Border,  rounded corners=3pt, line width=0.7pt] (30,660) rectangle (44,674);
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (50,667) {Node boundary};

\draw[fill=skelFill,   draw=skelBorder,   rounded corners=3pt, line width=0.7pt] (168,660) rectangle (182,674);
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (188,667) {Skeleton coordinator};

\draw[fill=stubFill,   draw=stubBorder,   rounded corners=3pt, line width=0.7pt] (340,660) rectangle (354,674);
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (360,667) {Stub coordinator};

\draw[fill=plugLdrFill, draw=plugLdrBorder, rounded corners=3pt, line width=0.7pt] (490,660) rectangle (504,674);
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (510,667) {Plugin ranks};

\draw[fill=gpuPlugFill, draw=gpuPlugBorder, rounded corners=3pt, line width=0.7pt] (630,660) rectangle (644,674);
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (650,667) {GPU / NCCL runtime};

%% Row 2 swatches
\draw[fill=gpuMonFill, draw=gpuMonBorder,  rounded corners=3pt, line width=0.7pt] (30,686) rectangle (44,700);
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (50,693) {GPU monitor (NVML)};

\draw[fill=shmFill, draw=shmBorder, dashed, rounded corners=3pt, line width=0.8pt] (206,686) rectangle (220,700);
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (226,693) {Shared memory (SHM)};

\draw[fill=agent2Fill, draw=agent2Border,  rounded corners=3pt, line width=0.7pt] (390,686) rectangle (404,700);
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (410,693) {Agent-2-OCS (config selector)};

\draw[fill=agent1Fill, draw=agent1Border,  rounded corners=3pt, line width=0.7pt] (610,686) rectangle (624,700);
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (630,693) {Agent-1-CD (contention detector)};

%% Divider
\draw[arrowNccl, line width=0.7pt] (30,710) -- (870,710);
\node[font=\sffamily\bfseries\scriptsize, text=textDark, anchor=west] at (30,726) {Control flow};

%% Step badges row 1
\node[stepbadge, fill=arrowOrange, minimum size=20pt] at (118,726) {1};
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (133,726) {DDP invokes collective};

\node[stepbadge, fill=arrowRed,    minimum size=20pt] at (290,726) {2};
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (305,726) {GPU telemetry $\to$ SHM};

\node[stepbadge, fill=arrowOrange, minimum size=20pt] at (460,726) {3};
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (475,726) {Coordinator reads SHM + collInfo};

\node[stepbadge, fill=arrowGreen,  minimum size=20pt] at (670,726) {4};
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (685,726) {Agents detect + select config};

%% Step badges row 2
\node[stepbadge, fill=arrowGreen,  minimum size=20pt] at (118,754) {5};
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (133,754) {MPI\_Bcast config to all stubs};

\node[stepbadge, fill=arrowBlue,   minimum size=20pt] at (310,754) {6};
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (325,754) {Stubs inject config to ranks via TCP};

\node[stepbadge, fill=arrowGray,   minimum size=20pt] at (530,754) {7};
\node[font=\sffamily\scriptsize, text=textMid, anchor=west] at (545,754) {NCCL applies config to collective op};

\end{tikzpicture}

==> sections/psudocode/optimizer_pseudocode.tex <==
\begin{algorithm}[t]
\caption{Optimizer -- Critical Path}
\label{alg:optimizer}
\begin{algorithmic}[1]

\small
\Statex \textbf{Input:} collInfo ($nRanks, nNodes, collType, nBytes$)
\Statex \textbf{Output:} Config (A, P, nCh, nTh)

\State key $\gets$ (collInfo.$collType$, collInfo.$nBytes$)\Comment{unique pair}
\If{key in KV\_Cache} \Comment{mutex-protected operation}
    \State \Return KV\_Cache[key] \Comment{O(1) hash lookup}
\ElsIf{key in cold\_start\_configs} \Comment{If Preloaded}
    \State cfg $\gets$ cold\_start\_configs[key]
\Else
    \State cfg $\gets$ (Ring, Simple, 1, 512) \Comment{fallback default}
\EndIf
\State KV\_Cache[key] $\gets$ cfg \Comment{populate for future hits}
\State \Return cfg

\end{algorithmic}
\end{algorithm}



==> sections/tables/symbol_table.tex <==
%% Notation Table for DynamICCL
\begin{table}[t]
\centering
\caption{Summary of notation used throughout this paper.}
\label{tab:notation}
\small
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{@{}lp{0.62\linewidth}@{}}
\toprule
\textbf{Symbol} & \textbf{Description} \\
\midrule
\multicolumn{2}{@{}l}{\textit{NCCL Configuration Tuple}} \\
$\mathcal{A}_{\text{algo}}$ & Algorithm dimension: $\{\text{Ring}, \text{Tree}\}$ \\
$\mathcal{P}$               & Protocol dimension: $\{\text{LL}, \text{Simple}\}$ \\
$n_{\text{Ch}}$             & Number of channels (link parallelism): $\{1,\dots,8\}$ \\
$n_{\text{Th}}$             & Number of threads: $\{128, 256, 512\}$ \\
$(c, b)$                    & Collective key: $(collType,\ nBytes)$ used to index KV cache \\
\midrule
\multicolumn{2}{@{}l}{\textit{Agent-1: Contention Detection (\agentone{})}} \\
$t$                         & Discrete iteration index (one collective call observation) \\
$L_{\text{obs}}$            & Observed AllReduce latency at iteration $t$ \\
$L_{\text{baseline}}$       & Median latency under zero contention for key $(c, b)$ \\
$r_t$                       & Contention ratio: $L_{\text{obs}} / L_{\text{baseline}}$ \\
$\mathbf{u}_t$              & 15-dimensional LSTM input vector at iteration $t$ \\
$(h_t,\ c_t)$               & LSTM hidden and cell state carried across iterations \\
$p_t$                       & Posterior probability of SUSTAINED contention: $P(\text{SUSTAINED} \mid \mathbf{u}_{1:t})$ \\
$\tau_U,\ \tau_L$           & SPRT upper and lower decision thresholds (0.95 and 0.05) \\
$a_t$                       & \agentone{} output: SUSTAINED, SPIKE, or WAIT \\
$\mathbf{c}_t$              & Contention vector forwarded to \agenttwo{}: $[\text{dir}, \text{mag}, \text{conf}]$ \\
\midrule
\multicolumn{2}{@{}l}{\textit{Agent-2: Configuration Selection (\agenttwo{})}} \\
$(S, \mathcal{A}, R, P)$    & MDP tuple: states, actions, reward signal, transition dynamics \\
$\mathbf{s}$                & 153-dimensional state vector: 25 base features $+$ 128-dim $h_t$ \\
$L_{\text{zero-best}}$      & Best observed latency under zero contention for key $(c, b)$ \\
$r$                         & Reward signal: $(L_{\text{zero-best}} - L_{\text{obs}}) / L_{\text{zero-best}} \leq 0$ \\
$\theta,\ \theta^-$         & Online and target network parameters \\
$\gamma$                    & Discount factor \\
$d$                         & Terminal state indicator \\
$y$                         & Double DQN Bellman target \\
$V(\mathbf{s})$             & Value stream output: estimated quality of state $\mathbf{s}$ \\
$\Phi(\mathbf{s}, a)$       & Advantage stream output: relative benefit of action $a$ in state $\mathbf{s}$ \\
$Q(\mathbf{s}, a)$          & Q-value: $V(\mathbf{s}) + \Phi(\mathbf{s},a) - \frac{1}{|\mathcal{A}|}\sum_{a'}\Phi(\mathbf{s},a')$ \\
$\mathcal{L}_{\text{Bell}}$ & Huber-based Bellman loss \\
$\mathcal{L}_{\text{CQL}}$  & Conservative Q-Learning regularization loss \\
$\alpha_{\text{CQL}}$       & CQL regularization coefficient (0.001) \\
\midrule
\multicolumn{2}{@{}l}{\textit{Coordinator Architecture}} \\
$R$                         & Number of NCCL ranks on a node \\
$C,\ C'$                    & Current and updated NCCL configuration tuple $(\mathcal{A}_{\text{algo}}, \mathcal{P}, n_{\text{Ch}}, n_{\text{Th}})$ \\
\bottomrule
\end{tabular}
\end{table}
